Bootstrapping Autonomous Driving Radars with Self-Supervised Learning

The perception of autonomous vehicles using radars has attracted increased research interest due its ability to operate in fog and bad weather. However, training radar models is hindered by the cost and difficulty of annotating large-scale radar data. To overcome this bottleneck, we propose a self-supervised learning framework to leverage the large amount of unlabeled radar data to pre-train radar-only embeddings for self-driving perception tasks. The proposed method combines radar-to-radar and radar-to-vision contrastive losses to learn a general representation from unlabeled radar heatmaps paired with their corresponding camera images. When used for downstream object detection, we demonstrate that the proposed self-supervision framework can improve the accuracy of state-of-the-art supervised baselines by $5.8\%$ in mAP. Code is available at \url{https://github.com/yiduohao/Radical}.

==> tex/ablationTab-2.tex <==
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\begin{table*}[h!]
\begin{minipage}[t]{0.95\linewidth}
    \centering
    \setlength{\tabcolsep}{8pt}
    \resizebox{0.95\linewidth}{!}
    {
        \begin{tabular}{l|cccccccc}
           Method & $\operatorname{AP}$ & $\operatorname{AP}_{50}$ & $\operatorname{AP}_{75}$ & $\operatorname{AP}_{str}$ & $\operatorname{AP}_{ori}$ & $\operatorname{AP}_{inc}$  \\
            \hline
            Rotation & $61.4 \pm 0.6$ & $89.0\pm0.6$ & $68.7\pm1.0$ & $68.0\pm0.7$ & $32.0\pm0.7$ & $31.2\pm1.9$ \\
            Center Crop & $61.0 \pm 1.0$ & $89.2\pm0.7$ & $67.7\pm1.4$ & $67.2\pm0.9$ & $33.2\pm1.9$ & $32.5\pm2.4$ \\
            Random Weights & $60.8 \pm 0.5$ & $89.4\pm0.4$ & $68.3\pm0.9$ & $67.0\pm0.5$ & $32.7\pm1.3$ & $32.7\pm1.1$ \\
            Horizontal Flip & $59.6 \pm 0.8$ & $89.0\pm0.3$ & $67.5\pm1.3$ & $65.9\pm1.0$ & $31.8\pm1.7$ & $30.2\pm1.3$ \\
            \hline
            Cross-modal Only & $60.0 \pm 0.6$ & $88.9 \pm 0.2$ & $66.9 \pm 0.9$ & $66.2 \pm 0.5$ & $31.4 \pm 1.0$ & $31.4\pm1.6$ \\
            \hline
            Threshold & $59.5 \pm 0.6$ & $88.7\pm0.5$ & $66.4\pm1.1$ & $65.6\pm0.7$ & $32.0\pm2.1$ & $30.7\pm1.5$ \\
            Cutout & $58.4 \pm 1.2$ & $89.0\pm0.5$ & $66.8\pm1.2$ & $64.2\pm1.4$ & $32.1\pm1.1$ & $31.6\pm1.8$ \\
            Vertical Flip & $58.1 \pm 0.6$ & $88.5\pm0.3$ & $66.6\pm0.9$ & $64.0\pm0.8$ & $32.4\pm1.1$ & $30.8\pm1.2$ \\
        \end{tabular}
    }
    \caption{\textbf{Effect of adding augmentation on the baseline. BEV rotated bounding box object detection results on Radatron dataset} For row 1, the backbone of the detection model is randomly initialized. For row 2, 3 and 4, we pre-trained the model with 63k Radatron unlabeled frames, and fine-tuned it on 13k Radatron labeled frames. Results are averaged for 6 runs.}
    \label{tab:ablate:grad_add}
\end{minipage}
\vspace{2mm}
\end{table*}


\begin{table*}[t]
\centering

\begin{tabular}{cccc|cccccc}
   RW & CC & HF & ROT & AP & AP$_{50}$ & AP$_{75}$ & AP$_{str}$ & AP$_{ori}$ & AP$_{inc}$ \\
    \hline
   \cmark & \cmark & \cmark & \cmark & $60.9 \pm 0.5$ & $89.1 \pm 0.4$ & $67.7 \pm 0.9$ & $67.8 \pm 0.4$ & $31.7 \pm 0.8$ & $31.9 \pm 1.8$ \\
   \xmark & \cmark & \cmark & \cmark & $59.4 \pm 1.1$ & $88.8 \pm 0.4$ & $67.2 \pm 1.5$ & $65.6 \pm 1.1$ & $30.1 \pm 2.6$ & $31.7 \pm 1.6$  \\
   \cmark & \xmark & \cmark & \cmark & $60.4 \pm 0.6$ & $88.9 \pm 0.5$ & $67.2 \pm 1.0$ & $66.7 \pm 0.9$ & $31.3 \pm 1.4$ & $31.7 \pm 1.5$ \\
   \cmark & \cmark & \xmark & \cmark & $59.4 \pm 1.0$ & $89.3 \pm 0.4$ & $67.6 \pm 0.9$ & $65.2 \pm 1.2$ & $32.7 \pm 1.1$ & $31.9 \pm 2.3$  \\
   \cmark & \cmark & \cmark & \xmark & \bf{62.3}$\pm0.6$ & \bf{89.6}$\pm0.1$ & \bf{69.7}$\pm1.2$ & \bf{68.7}$\pm0.5$ & \bf{33.0}$\pm1.5$ & $31.8\pm1.3$ \\
\end{tabular}

\caption{\textbf{Effect of removing each augmentation from our method. BEV rotated bounding box object detection results on Radatron dataset} For row 1, the backbone of the detection model is randomly initialized. For row 2, 3 and 4, we pre-trained the model with 63k Radatron unlabeled frames, and fine-tuned it on 13k Radatron labeled frames. Results are averaged for 6 runs.}
\label{tab:ablate:remove_each}

% \vspace{3mm}
% \subfloat[Effect of Adding two augmentations
% \label{tab:ablate:two_aug}
% ]{
% \centering
% \begin{minipage}{1\linewidth}{\begin{center}
% \resizebox{0.75\linewidth}{!}
% {
% \begin{tabular}{cccc|cccccc}
%    RW & CC & HF & THR & AP & AP$_{50}$ & AP$_{75}$ & AP$_{str}$ & AP$_{ori}$ & AP$_{inc}$ \\
%     \hline
%    \cmark & \cmark & \xmark & \xmark & $61.7 \pm 0.5$ & $89.5 \pm 0.4$ & $68.5 \pm 1.0$ & $67.9 \pm 0.7$ & $34.0 \pm 1.1$ & $33.0 \pm 1.8$ \\
%    \cmark & \xmark & \cmark & \xmark & $59.8 \pm 0.7$ & $ $ & $ $ & $ $ & $ $ & $ $ \\
%    \cmark & \xmark & \xmark & \cmark & $60.3 \pm 0.6$ & $ $ & $ $ & $ $ & $ $ & $ $ \\
%    \xmark & \cmark & \cmark & \xmark & $61.9 \pm 0.7$ & $89.7 \pm 0.3$ & $68.9 \pm 1.1$ & $68.0 \pm 0.7$ & $32.9 \pm 1.5$ & $32.7 \pm 1.2$ \\
%    \xmark & \cmark & \xmark & \cmark & $59.9 \pm 1.0$ & $ $ & $ $ & $ $ & $ $ & $ $ \\
%    \xmark & \xmark & \cmark & \cmark & $59.9 \pm 0.7$ & $ $ & $ $ & $ $ & $ $ & $ $ \\
% \end{tabular}
% }
% \end{center}}
% \end{minipage}
% }
\vspace{2mm}
\caption{\textbf{Ablation experiments on different augmentation methods based on Radatron} RW: random weights. CC: center crop. HF: horizontal flip. VF: vertical flip. THR: thresholding. CUT: cutout. ROT: rotation. All experiments are based on Intra+Cross Modal with CimCLR+SYM3 implementation.}
\label{tab:ablate_group_1}
\end{table*}

==> tex/mainTab-2.tex <==
\begin{table}[h!]
\begin{minipage}[t]{\linewidth}
    \centering
    \setlength{\tabcolsep}{8pt}
    \resizebox{\linewidth}{!}
    {
        \begin{tabular}{l|ccccc}
           Method & $\operatorname{AP}$ & $\operatorname{AP}_{50}$ & $\operatorname{AP}_{75}$ \\
            \hline
           Random Initialization & $56.5\pm0.2$ & $88.9\pm0.4$ & $64.5\pm1.7$ \\ 
           Intra-modal (SimCLR) + Aug. & $59.4\pm1.0$ & $89.1\pm0.5$ & $66.8\pm1.8$ \\ 
           Cross-modal (MoCo v2) & $59.9\pm1.0$ & $89.1\pm0.2$ & $67.5\pm0.4$ \\ 
           Cross-modal (SimCLR) & $59.9\pm0.6$ & $88.9\pm0.2$ & $66.9\pm0.9$ \\ 
           Intra+Cross (SimCLR) + Aug. & \bf{62.3}$\pm0.6$ & \bf{89.6}$\pm0.1$ & \bf{69.7}$\pm1.2$ \\ 
        \end{tabular}
    }
    \caption{\textbf{BEV rotated bounding box object detection results on Radatron dataset} For row 1, the backbone of the detection model is randomly initialized. For row 2, 3 and 4, we pre-trained the model with 32k Radatron unlabeled frames, and fine-tuned it on 13k Radatron labeled frames. Results are averaged for 6 runs.}
    \label{tab:exp_radatron_ft}
\end{minipage}
\vspace{2mm}

\begin{minipage}[t]{\linewidth}
    \centering
    \setlength{\tabcolsep}{8pt}
    \resizebox{\linewidth}{!}
    {
        \begin{tabular}{l|ccccc}
           Method & $\operatorname{AP}$ & $\operatorname{AP}_{50}$ & $\operatorname{AP}_{75}$ \\
            \hline
           Random Initialization & $22.1\pm0.8$ & $48.0\pm1.5$ & $17.7\pm1.2$ \\ 
           Intra-modal (SimCLR) + Aug. & $45.4 \pm 0.1$ & $78.3\pm0.1$ & $48.6\pm0.5$ \\ 
           Cross-modal (MoCo v2) & $49.9\pm0.1$ & $84.7\pm0.1$ & $56.1\pm0.3$ \\ 
           Cross-modal (SimCLR) & $46.3\pm0.1$ & $83.0\pm0.1$ & $49.4\pm0.3$ \\ 
           Intra+Cross (SimCLR) + Aug. & \bf{52.6}$\pm0.1$ & \bf{86.9}$\pm0.1$ & \bf{58.5}$\pm0.2$ \\ 
        \end{tabular}
    }
    \caption{\textbf{BEV rotated bounding box object detection results on Radatron dataset with frozen backbone} For row 1, the backbone of the detection model is randomly initialized and frozen during fine-tuning. For row 2, 3 and 4, we pre-trained the model with 32k Radatron unlabeled frames, and fine-tuned it with backbone frozen on 13k Radatron labeled frames. Results are averaged for 2 runs.}
    \label{tab:exp_radatron_ft}
\end{minipage}
\end{table}
